Program Synthesis in Saturation

We present an automated reasoning framework for synthesizing recursion-free programs using saturation-based theorem proving. Given a functional specification encoded as a first-order logical formula, we use a first-order theorem prover to both establish validity of this formula and discover program fragments satisfying the specification. As a result, when deriving a proof of program correctness, we also synthesize a program that is correct with respect to the given specification. We describe properties of the calculus that a saturation-based prover capable of synthesis should employ, and extend the superposition calculus in a corresponding way. We implemented our work in the first-order prover Vampire, extending the successful applicability of first-order proving to program synthesis. This is an extended version of an Automated Deduction -- CADE 29 paper with the same title and the same authors.

==> simplification.tex <==
\PH{I'd propose moving all this to the end of Section~\ref{sec:synth-with-al}.}

When constructing the final program from the set $\mathcal{P}$, we do not simply use all programs of $\mathcal{P}$ as branches of one nested $\itecons$.
Rather, we simplify the program as follows.

First, as mentioned in Section~\ref{sec:synth-with-al}, we only use a program with conditions recorded during the proof search if the condition appears in the derivation of $\square$.
The reasoning for this is that we are looking for conditions $C_1[\overline{x}],\dots,C_n[\overline{x}]$ for the cases of our nested $\itecons$ as in~\eqref{eq:prog-construction} such that $\bigwedge_{i=1}^n A_i\land\bigwedge_{i=1}^k C_i[\overline{x}]$ is unsatisfiable.
That we can guarantee by selecting only those programs from $\mathcal{P}$ whose conditions occur in the derivation of $\square$.
Since these conditions cover all possible cases, we do not need to use any other programs from $\mathcal{P}$.

Second, if we recorded a program $\langle z, C\rangle$ where $z$ is a variable and $C$ is any condition, %then we use it in the final program construction only if all other recorded programs also correspond to a variable
we do not use it in the final program construction (see Example~\ref{ex:inv2}).
\PH{If we move this to the end of Section~\ref{sec:synth-with-al}, remove the reference to Example, and rather refer to this text from the Example.}
This is because $z$ represents an arbitrary witness -- therefore any other program $\langle t, C'\rangle$ (where $t$ is not a variable) computes a satisfactory witness for the condition $C$.
If all recorded programs correspond to a variable, then we choose a constant of the corresponding sort, and use that as the final program.

We could also employ simplification in the style of \PH{TODO: the simplification techniques from interpolation?}.

Another option is to utilize the simplification rules of the theorem prover.
In the saturation loop of Algorithm~\ref{alg:saturation-new} we can first simplify clause $C_i$, and only then carry out the program recording and answer literal removal on lines 6-10.
%In practice we need to be careful with such simplification so that we do not modify the answer literal in $C_i$.
%\PH{Do we though?}
\PH{This is what we can do easily (and it's pretty much implemented, I'd just have to move one block of code to a different place in the saturation algorithm).
Since we don't have the interpolation-style technique implemented, I would actually go with this. Thoughts?}
